Lighting-aware Unified Model for Instance Segmentation

Foundation models like the Segment Anything Model (SAM) demonstrate impressive zero-shot generalization but frequently degrade under diverse real-world illumination, particularly for instance segmentation. In this work, we address this limitation by developing Lighting Convolutional-Attention (LCA), an adapter module that enhances segmentation robustness without fine-tuning the heavy backbone. LCA employs a dual-branch architecture to process RGB features alongside contrast maps, enabling physically motivated sensitivity to structural changes rather than illumination artifacts. We optimize LCA through a pairwise training strategy, introducing a targeted loss term that explicitly penalizes discrepancies between clean images and their corresponding illumination variants. To evaluate and support this architecture, we conduct a comprehensive empirical study across multiple existing benchmarks and present a novel Unity-based synthetic dataset specifically designed to accurately replicate complex real-world lighting conditions. Extensive experimental results demonstrate that our approach successfully bridges the domain gap, delivering superior lighting-robust segmentation.

==> tables_new/T10_severity_main.tex <==
\begin{table}[t]
\centering
\caption{\revised{Relative mIoU degradation at severity~3, $100\cdot(\text{clean}-\text{sev3})/\text{clean}$;
lower is better. Absolute gaps are not comparable across models, since a model sitting lower on
clean has less to lose. \lca{}+Dec degrades least on all four core datasets. Absolute scores
at every severity, on all five datasets and four metrics: \tableref{tab:severity_full}.}}
\label{tab:severity_main}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}l|cccc@{}}
\toprule
\revised{Dataset} & \revised{SAM} & \revised{Dec} & \revised{\lca{}} & \revised{\lca{}+Dec} \\
\midrule
\revised{Cityscapes} & \revised{1.87} & \revised{0.95} & \revised{0.76} & \revised{\textbf{0.74}} \\
\revised{COCO}       & \revised{1.76} & \revised{0.90} & \revised{0.96} & \revised{\textbf{0.83}} \\
\revised{VOC}        & \revised{1.80} & \revised{2.33} & \revised{1.82} & \revised{\textbf{1.69}} \\
\revised{Unity}      & \revised{1.02} & \revised{1.10} & \revised{1.07} & \revised{\textbf{0.91}} \\
\bottomrule
\end{tabular}
\end{table}


==> tables_new/T11_transfer.tex <==
\begin{table}[t]
\centering
\caption{\revised{Synthetic-to-real transfer. \lca{}+Dec on SAM~3 is trained on COCO with
\plap{} and evaluated on real ACDC imagery with \emph{no ACDC gradient steps}; checkpoints
were selected on COCO val. mIoU on the unmodified ACDC photograph, mean\,$\pm$\,population sd
over three seeds. Both columns score the same instances, so $\Delta$ is paired.}}
\label{tab:transfer}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}l|cc|c|c@{}}
\toprule
\revised{Condition} & \revised{SAM~3} & \revised{+\lca{}+Dec} & \revised{$\Delta$} & \revised{Inst.} \\
\midrule
\revised{Fog}   & \revised{0.7393} & \revised{\textbf{0.8212}\,{\tiny$\pm$.0070}} & \revised{\textbf{+0.0819}} & \revised{643} \\
\revised{Night} & \revised{0.6623} & \revised{\textbf{0.7431}\,{\tiny$\pm$.0031}} & \revised{\textbf{+0.0808}} & \revised{558} \\
\revised{Rain}  & \revised{0.6961} & \revised{\textbf{0.7777}\,{\tiny$\pm$.0072}} & \revised{\textbf{+0.0816}} & \revised{763} \\
\revised{Snow}  & \revised{0.7027} & \revised{\textbf{0.8021}\,{\tiny$\pm$.0084}} & \revised{\textbf{+0.0994}} & \revised{829} \\
\bottomrule
\end{tabular}
\end{table}


==> tables_new/T2_compact.tex <==
\begin{table*}[t]
\centering
\caption{%
  \revised{Main results. \textbf{C}\,=\,Clean, \textbf{V}\,=\,Lighting variant.
  Each backbone is placed beside the same backbone carrying \lca{} and a tuned mask
  decoder, so each pair isolates what the adapter adds to that encoder. \lca{} columns
  are mean\,$\pm$\,population sd over three seeds.
  \textbf{Bold}: best per row and stream. The SAM, SAM~2.1, decoder-only and
  \lca{}-only configurations, and the four ACDC conditions, are in the appendix
  (\tableref{tab:t2full_miou}).}
  $^{\dagger}$YOLOv11s mIoU (C/V): City 0.245/0.238, COCO 0.364/0.346,
  VOC 0.542/0.518, Unity 0.052/0.038; mask AP not evaluated.
}
\label{tab:main_results}
\footnotesize
\renewcommand{\arraystretch}{0.9}
\setlength{\tabcolsep}{2pt}
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{tabularx}{\linewidth}{ll|YY|YY|YY|YY}
\toprule
 & & \multicolumn{2}{c|}{HQ-SAM} & \multicolumn{2}{c|}{\textbf{HQ-SAM+\lca{}}} & \multicolumn{2}{c|}{SAM\,3} & \multicolumn{2}{c}{\textbf{SAM\,3+\lca{}}} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
\textbf{Metric} & \textbf{Dataset} & \textbf{C} & \textbf{V} & \textbf{C} & \textbf{V} & \textbf{C} & \textbf{V} & \textbf{C} & \textbf{V} \\
\midrule
\multirow{4}{*}{mIoU}
  & Cityscapes & 0.4737 & 0.4713 & \textbf{0.7851}{\tiny$\pm$.0006} & \textbf{0.7820}{\tiny$\pm$.0008} & 0.6496 & 0.6486 & 0.7662{\tiny$\pm$.0042} & 0.7634{\tiny$\pm$.0042} \\
  & COCO & 0.6585 & 0.6539 & 0.8178{\tiny$\pm$.0011} & 0.8153{\tiny$\pm$.0012} & 0.7607 & 0.7602 & \textbf{0.8207}{\tiny$\pm$.0006} & \textbf{0.8196}{\tiny$\pm$.0006} \\
  & VOC & 0.6131 & 0.6078 & 0.7561{\tiny$\pm$.0012} & 0.7498{\tiny$\pm$.0012} & 0.6918 & 0.6909 & \textbf{0.7873}{\tiny$\pm$.0015} & \textbf{0.7838}{\tiny$\pm$.0014} \\
  & Unity & 0.6047 & 0.6018 & \textbf{0.8816}{\tiny$\pm$.0017} & \textbf{0.8722}{\tiny$\pm$.0003} & 0.7325 & 0.7284 & 0.8679{\tiny$\pm$.0007} & 0.8591{\tiny$\pm$.0004} \\
\midrule
\multirow{4}{*}{pmAP$_{50}$}
  & Cityscapes & 0.5224 & 0.5166 & \textbf{0.9143}{\tiny$\pm$.0026} & \textbf{0.9112}{\tiny$\pm$.0021} & 0.7623 & 0.7627 & 0.9076{\tiny$\pm$.0053} & 0.9030{\tiny$\pm$.0090} \\
  & COCO & 0.7751 & 0.7692 & \textbf{0.9674}{\tiny$\pm$.0011} & 0.9661{\tiny$\pm$.0003} & 0.9264 & 0.9242 & 0.9663{\tiny$\pm$.0004} & \textbf{0.9666}{\tiny$\pm$.0010} \\
  & VOC & 0.6952 & 0.6841 & 0.8653{\tiny$\pm$.0006} & 0.8578{\tiny$\pm$.0027} & 0.7930 & 0.7927 & \textbf{0.9000}{\tiny$\pm$.0018} & \textbf{0.8939}{\tiny$\pm$.0025} \\
  & Unity & 0.6427 & 0.6398 & \textbf{0.9493}{\tiny$\pm$.0022} & \textbf{0.9440}{\tiny$\pm$.0018} & 0.8192 & 0.8177 & 0.9358{\tiny$\pm$.0004} & 0.9303{\tiny$\pm$.0028} \\
\midrule
\multirow{4}{*}{pmAP$_{75}$}
  & Cityscapes & 0.2483 & 0.2412 & \textbf{0.6782}{\tiny$\pm$.0048} & \textbf{0.6718}{\tiny$\pm$.0044} & 0.4049 & 0.4053 & 0.6262{\tiny$\pm$.0057} & 0.6213{\tiny$\pm$.0070} \\
  & COCO & 0.4512 & 0.4399 & 0.7790{\tiny$\pm$.0031} & 0.7695{\tiny$\pm$.0026} & 0.6342 & 0.6389 & \textbf{0.7895}{\tiny$\pm$.0026} & \textbf{0.7873}{\tiny$\pm$.0020} \\
  & VOC & 0.4339 & 0.4313 & 0.6410{\tiny$\pm$.0010} & 0.6328{\tiny$\pm$.0024} & 0.5948 & 0.5916 & \textbf{0.6945}{\tiny$\pm$.0053} & \textbf{0.6895}{\tiny$\pm$.0045} \\
  & Unity & 0.4399 & 0.4447 & \textbf{0.8569}{\tiny$\pm$.0040} & \textbf{0.8408}{\tiny$\pm$.0013} & 0.6202 & 0.6088 & 0.8360{\tiny$\pm$.0023} & 0.8259{\tiny$\pm$.0017} \\
\midrule
\multirow{4}{*}{pmAP}
  & Cityscapes & 0.2757 & 0.2711 & \textbf{0.6417}{\tiny$\pm$.0004} & \textbf{0.6356}{\tiny$\pm$.0008} & 0.4244 & 0.4222 & 0.6097{\tiny$\pm$.0077} & 0.6052{\tiny$\pm$.0080} \\
  & COCO & 0.4473 & 0.4404 & 0.6934{\tiny$\pm$.0018} & 0.6882{\tiny$\pm$.0019} & 0.5895 & 0.5894 & \textbf{0.7007}{\tiny$\pm$.0008} & \textbf{0.6984}{\tiny$\pm$.0008} \\
  & VOC & 0.4318 & 0.4244 & 0.6123{\tiny$\pm$.0013} & 0.6019{\tiny$\pm$.0021} & 0.5584 & 0.5563 & \textbf{0.6606}{\tiny$\pm$.0023} & \textbf{0.6549}{\tiny$\pm$.0025} \\
  & Unity & 0.4356 & 0.4328 & \textbf{0.8264}{\tiny$\pm$.0034} & \textbf{0.8089}{\tiny$\pm$.0006} & 0.5935 & 0.5862 & 0.8043{\tiny$\pm$.0012} & 0.7903{\tiny$\pm$.0012} \\
\bottomrule
\end{tabularx}
\end{table*}


==> tables_new/T3_compute.tex <==
\begin{table}[t]
\centering
\caption{\revised{Deployment cost. Median of 100 iterations after 20 warm-up iterations,
fp16, batch~1 at $1024{\times}1024$, one RTX~4090; \textbf{IQR} is the interquartile range
over those iterations, so every median is separated far beyond the measurement spread.
\textbf{Params} counts the image encoder, where \lca{} is inserted; the encoder is frozen in every configuration, and only the adapter and the mask decoder (4.06\,M) receive gradients. Memory is
activation memory, not weight memory.}}
\label{tab:compute_main}
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}l|ccccc@{}}
\toprule
\revised{Model} & \revised{Params} & \revised{GFLOPs} & \revised{Lat.} & \revised{IQR} & \revised{Mem.} \\
 & \revised{(M)} & & \revised{(ms)} & \revised{(ms)} & \revised{(MB)} \\
\midrule
\revised{SAM}                & \revised{89.67}  & \revised{486.4}  & \revised{28.27} & \revised{0.13} & \revised{1388.2} \\
\revised{~~+ \lca{}}         & \revised{92.17}  & \revised{496.3}  & \revised{31.63} & \revised{0.11} & \revised{1399.2} \\
\revised{~~+ \lca{}+Dec}     & \revised{95.66}  & \revised{511.0}  & \revised{30.54} & \revised{0.08} & \revised{1406.3} \\
\midrule
\revised{HQ-SAM}             & \revised{89.67}  & \revised{486.4}  & \revised{28.17} & \revised{0.03} & \revised{1406.2} \\
\revised{~~+ \lca{}+Dec}     & \revised{95.66}  & \revised{511.0}  & \revised{30.41} & \revised{0.03} & \revised{1424.3} \\
\midrule
\revised{SAM~3}              & \revised{454.04} & \revised{2806.7} & \revised{52.82} & \revised{0.02} & \revised{1114.6} \\
\revised{~~+ \lca{}+Dec}     & \revised{464.65} & \revised{2861.6} & \revised{57.65} & \revised{0.03} & \revised{1136.6} \\
\bottomrule
\end{tabular}
\end{table}


==> tables_new/T4_resolution_full.tex <==
\begin{table*}[t]
\centering
\caption{\revised{Input-resolution sweep on VOC, full grid. \textbf{Data axis}: the loader decodes at $S{\times}S$ and the image is upsampled back to the encoder's native 1024, so the encoder always receives $64{\times}64=4{,}096$ tokens. \textbf{Encoder axis}: the encoder's input really is $S{\times}S$, the token grid shrinks accordingly and the position embedding is interpolated, with the loader pinned at 512. Validation resolution is fixed, so every row scores the same 3{,}406 instances against the same ground truth. \textbf{C}/\textbf{V} are the clean and lighting-variant streams; single run per cell. $^{*}$Encoder-axis 1024 is data-axis 512 by construction -- the same trained model -- so the axes meet there rather than agreeing by measurement.}}
\label{tab:resolution_full}
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{@{}llcccccccc@{}}
\toprule
 & & \multicolumn{4}{c}{\textbf{Data axis} (loader)} & \multicolumn{4}{c}{\textbf{Encoder axis} (encoder input)} \\
\cmidrule(lr){3-6}\cmidrule(lr){7-10}
 & & \multicolumn{2}{c}{SAM} & \multicolumn{2}{c}{+\lca{}} & \multicolumn{2}{c}{SAM} & \multicolumn{2}{c}{+\lca{}} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
\textbf{Metric} & \textbf{Size} & C & V & C & V & C & V & C & V \\
\midrule
\multirow{4}{*}{mIoU}
  & 128 & 0.5520 & 0.5472 & 0.7106 & 0.7047 & 0.3849 & 0.3772 & 0.5673 & 0.5628 \\
  & 256 & 0.6034 & 0.5984 & 0.7380 & 0.7317 & 0.5471 & 0.5423 & 0.6638 & 0.6605 \\
  & 512 & 0.6130 & 0.6076 & 0.7456 & 0.7380 & 0.6172 & 0.6122 & 0.7211 & 0.7175 \\
  & 1024$^{*}$ & 0.6108 & 0.6047 & 0.7429 & 0.7344 & 0.6130 & 0.6076 & 0.7456 & 0.7380 \\
\midrule
\multirow{4}{*}{pmAP$_{50}$}
  & 128 & 0.6124 & 0.6066 & 0.8095 & 0.8027 & 0.3453 & 0.3324 & 0.6289 & 0.6236 \\
  & 256 & 0.6794 & 0.6753 & 0.8406 & 0.8332 & 0.5887 & 0.5769 & 0.7355 & 0.7317 \\
  & 512 & 0.6935 & 0.6861 & 0.8503 & 0.8417 & 0.6870 & 0.6820 & 0.8206 & 0.8136 \\
  & 1024$^{*}$ & 0.6944 & 0.6835 & 0.8447 & 0.8353 & 0.6935 & 0.6861 & 0.8503 & 0.8417 \\
\midrule
\multirow{4}{*}{pmAP$_{75}$}
  & 128 & 0.3306 & 0.3250 & 0.5681 & 0.5578 & 0.1609 & 0.1550 & 0.3647 & 0.3529 \\
  & 256 & 0.4237 & 0.4143 & 0.6130 & 0.6016 & 0.3600 & 0.3541 & 0.5038 & 0.4982 \\
  & 512 & 0.4383 & 0.4281 & 0.6312 & 0.6169 & 0.4595 & 0.4533 & 0.6025 & 0.5919 \\
  & 1024$^{*}$ & 0.4336 & 0.4240 & 0.6318 & 0.6195 & 0.4383 & 0.4281 & 0.6312 & 0.6169 \\
\midrule
\multirow{4}{*}{pmAP}
  & 128 & 0.3414 & 0.3352 & 0.5417 & 0.5321 & 0.1754 & 0.1680 & 0.3653 & 0.3583 \\
  & 256 & 0.4210 & 0.4138 & 0.5840 & 0.5733 & 0.3566 & 0.3518 & 0.4858 & 0.4805 \\
  & 512 & 0.4356 & 0.4267 & 0.5973 & 0.5853 & 0.4459 & 0.4407 & 0.5698 & 0.5619 \\
  & 1024$^{*}$ & 0.4312 & 0.4222 & 0.5957 & 0.5831 & 0.4356 & 0.4267 & 0.5973 & 0.5853 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables_new/T4_resolution_main.tex <==
\begin{table}[t]
\centering
\caption{\revised{Input-resolution sweep on VOC, mIoU. \textbf{Data axis}: the loader decodes at $S{\times}S$ and the image is upsampled back to 1024, so the encoder always receives $4{,}096$ tokens and no embedding is interpolated. \textbf{Encoder axis}: the encoder input is $S{\times}S$, so the token grid shrinks and the position embedding is interpolated. The submitted sweep resized the ground-truth masks with the images, scoring each row against a different ground truth; with the validation resolution fixed all rows score the same 3{,}406 instances and the non-monotonic result disappears. $^{*}$Encoder-axis 1024 is data-axis 512 by construction. AP metrics: \tableref{tab:resolution_ap}.}}
\label{tab:image_size_ablation}
\footnotesize
\setlength{\tabcolsep}{2.2pt}
\begin{tabular}{@{}l|cccc|cccc@{}}
\toprule
 & \multicolumn{4}{c|}{\revised{Data axis}} & \multicolumn{4}{c}{\revised{Encoder axis}} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
 & \multicolumn{2}{c}{\revised{SAM}} & \multicolumn{2}{c|}{\revised{+\lca{}}} & \multicolumn{2}{c}{\revised{SAM}} & \multicolumn{2}{c}{\revised{+\lca{}}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
\revised{Size} & \revised{C} & \revised{V} & \revised{C} & \revised{V} & \revised{C} & \revised{V} & \revised{C} & \revised{V} \\
\midrule
\revised{128} & \revised{0.5520} & \revised{0.5472} & \revised{0.7106} & \revised{0.7047} & \revised{0.3849} & \revised{0.3772} & \revised{0.5673} & \revised{0.5628} \\
\revised{256} & \revised{0.6034} & \revised{0.5984} & \revised{0.7380} & \revised{0.7317} & \revised{0.5471} & \revised{0.5423} & \revised{0.6638} & \revised{0.6605} \\
\revised{512} & \revised{0.6130} & \revised{0.6076} & \revised{0.7456} & \revised{0.7380} & \revised{0.6172} & \revised{0.6122} & \revised{0.7211} & \revised{0.7175} \\
\revised{1024$^{*}$} & \revised{0.6108} & \revised{0.6047} & \revised{0.7429} & \revised{0.7344} & \revised{0.6130} & \revised{0.6076} & \revised{0.7456} & \revised{0.7380} \\
\bottomrule
\end{tabular}
\end{table}


==> tables_new/T5_gates.tex <==
\begin{table}[t]
\centering
\caption{\revised{Gate composition: how the three gates are combined. VOC, \lca{}-only,
$N{=}4$, single run. Conjunctive fusion multiplies the three gate responses, so a feature
survives only where all three agree.}}
\label{tab:lsa_version_ablation}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}l|c|cc@{}}
\toprule
\revised{Design} & \revised{Params} & \revised{Clean} & \revised{Variant} \\
\midrule
\revised{Sequential gating}  & \revised{151\,K}  & \revised{0.6698} & \revised{0.6626} \\
\revised{Additive fusion}    & \revised{151\,K}  & \revised{0.6686} & \revised{0.6608} \\
\revised{\textbf{Conjunctive fusion}} & \revised{2.49\,M} & \revised{\textbf{0.7027}} & \revised{\textbf{0.6946}} \\
\bottomrule
\end{tabular}
\end{table}


==> tables_new/T5b_gate_ablation.tex <==
\begin{table}[t]
\centering
\caption{\revised{Gate ablation: one gate removed at a time from the three-gate module. VOC,
$N{=}4$, mean over three seeds, with paired $t$ against a protocol-matched three-gate
baseline sharing model, dataset, seeds, $\lambda_{\text{cons}}$ and epochs, and differing only
in the removed gate.}}
\label{tab:gate_ablation}
\footnotesize
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{@{}l|cc|cc@{}}
\toprule
 & \multicolumn{2}{c|}{\revised{Clean}} & \multicolumn{2}{c}{\revised{Variant}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
\revised{Configuration} & \revised{mIoU} & \revised{$\Delta$ ($t$)} & \revised{mIoU} & \revised{$\Delta$ ($t$)} \\
\midrule
\revised{Three gates}     & \revised{\textbf{0.7129}} & \revised{--} & \revised{\textbf{0.7056}} & \revised{--} \\
\revised{~~$-$ channel}   & \revised{0.7127} & \revised{$-$0.0001 ($-$0.2)} & \revised{0.7050} & \revised{$-$0.0007 ($-$0.9)} \\
\revised{~~$-$ spatial}   & \revised{0.7099} & \revised{$-$0.0030 ($-$1.4)} & \revised{0.7024} & \revised{$-$0.0032 ($-$1.7)} \\
\revised{~~$-$ Laplacian} & \revised{0.7058} & \revised{$\bm{-}$\textbf{0.0071} ($\bm{-}$\textbf{3.1})} & \revised{0.6989} & \revised{$\bm{-}$\textbf{0.0067} ($\bm{-}$\textbf{3.0})} \\
\bottomrule
\end{tabular}
\end{table}


==> tables_new/T6_loss.tex <==
\begin{table}[t]
\centering
\caption{\revised{Loss weights, VOC, \lca{}-only, single run per cell.
\textbf{(a)} The consistency weight $\lambda_{\text{cons}}$ has a clear optimum: the variant
stream gains $0.0051$ from $\lambda_{\text{cons}}{=}0$ to $5$, against $0.0022$ on clean, and
the model degrades sharply once the term dominates. \textbf{(b)} The supervised blend
$\lambda_{\text{sup}}$ is flat, because the consistency term already couples the two streams.
Adopted defaults in \textbf{bold}.}}
\label{tab:cons_weight_ablation}
\small
\setlength{\tabcolsep}{4pt}
\begin{minipage}[t]{0.48\linewidth}
  \centering
  \revised{\textbf{(a)}~$\lambda_{\text{cons}}$ (consistency)}\\[3pt]
  \begin{tabular}{@{}c|cc@{}}
  \toprule
  \revised{$\lambda_{\text{cons}}$} & \revised{Clean} & \revised{Variant} \\
  \midrule
  \revised{0}    & \revised{0.7030} & \revised{0.6941} \\
  \revised{0.1}  & \revised{0.7027} & \revised{0.6946} \\
  \revised{1}    & \revised{0.7013} & \revised{0.6949} \\
  \revised{\textbf{5}} & \revised{\textbf{0.7052}} & \revised{\textbf{0.6992}} \\
  \revised{10}   & \revised{0.7035} & \revised{0.6954} \\
  \revised{20}   & \revised{0.7036} & \revised{0.6972} \\
  \revised{100}  & \revised{0.6709} & \revised{0.6661} \\
  \revised{2000} & \revised{0.6477} & \revised{0.6429} \\
  \bottomrule
  \end{tabular}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\linewidth}
  \centering
  \revised{\textbf{(b)}~$\lambda_{\text{sup}}$ (supervised blend)}\\[3pt]
  \begin{tabular}{@{}c|cc@{}}
  \toprule
  \revised{$\lambda_{\text{sup}}$} & \revised{Clean} & \revised{Variant} \\
  \midrule
  \revised{0}   & \revised{0.6999} & \revised{0.6925} \\
  \revised{0.1} & \revised{0.7002} & \revised{0.6922} \\
  \revised{0.3} & \revised{0.6995} & \revised{0.6924} \\
  \revised{\textbf{0.5}} & \revised{\textbf{0.7004}} & \revised{\textbf{0.6922}} \\
  \revised{0.7} & \revised{0.7014} & \revised{0.6941} \\
  \revised{0.9} & \revised{0.7021} & \revised{0.6949} \\
  \revised{1}   & \revised{0.7026} & \revised{0.6954} \\
  \bottomrule
  \end{tabular}
\end{minipage}
\end{table}


==> tables_new/T9_nblocks.tex <==
\begin{table}[t]
\centering
\caption{\revised{Number of patched blocks $N$, VOC, \lca{}-only, mean\,$\pm$\,population sd
over three seeds. $N{=}0$ is the frozen backbone. Almost all of the gain arrives by $N{=}4$;
going to $N{=}10$ adds $0.0043$ clean mIoU for $2.5\times$ the parameters.}}
\label{tab:nblocks}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}c|c|cc@{}}
\toprule
\revised{$N$} & \revised{\lca{} params} & \revised{Clean} & \revised{Variant} \\
\midrule
\revised{0}   & \revised{--}      & \revised{0.6135} & \revised{0.6091} \\
\revised{2}   & \revised{1.25\,M} & \revised{0.6950\,{\tiny$\pm$.0058}} & \revised{0.6886\,{\tiny$\pm$.0045}} \\
\revised{\textbf{4}} & \revised{\textbf{2.49\,M}} & \revised{0.7029\,{\tiny$\pm$.0053}} & \revised{0.6947\,{\tiny$\pm$.0056}} \\
\revised{6}   & \revised{3.74\,M} & \revised{\textbf{0.7090}\,{\tiny$\pm$.0025}} & \revised{\textbf{0.7017}\,{\tiny$\pm$.0026}} \\
\revised{8}   & \revised{4.99\,M} & \revised{0.7079\,{\tiny$\pm$.0011}} & \revised{0.7011\,{\tiny$\pm$.0021}} \\
\revised{10}  & \revised{6.24\,M} & \revised{0.7072\,{\tiny$\pm$.0030}} & \revised{0.7000\,{\tiny$\pm$.0037}} \\
\bottomrule
\end{tabular}
\end{table}

